Evaluating Different Fault Injection Abstractions on the Assessment of DNN SW Hardening Strategies

The reliability of Neural Networks has gained significant attention, prompting efforts to develop SW-based hardening techniques for safety-critical scenarios. However, evaluating hardening techniques using application-level fault injection (FI) strategies, which are commonly hardware-agnostic, may yield misleading results. This study for the first time compares two FI approaches (at the application level (APP) and instruction level (ISA)) to evaluate deep neural network SW hardening strategies. Results show that injecting permanent faults at ISA (a more detailed abstraction level than APP) changes completely the ranking of SW hardening techniques, in terms of both reliability and accuracy. These results highlight the relevance of using an adequate analysis abstraction for evaluating such techniques.

==> tables/colored_complete_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{\todo{This caption is missing. Why wasn't the results of Lenet reported here?. There is something called FM that is not reported in the methodology or experimental setup}}
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{7}{c|}{\textbf{Mobilenet V2}} &
  \multicolumn{5}{c}{\textbf{Resnet 18}} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fault\\ model\end{tabular}}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hardening\\ Strategy\end{tabular}}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} &
  \multicolumn{4}{c}{\textbf{Bit Error Rate}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} &
  \multicolumn{4}{c}{Bit Error Rate} \\ \cline{4-7} \cline{9-12} 
 &
   &
   &
  \multicolumn{2}{c|}{$10^{-6}$} &
  \multicolumn{2}{c}{$10^{-5}$} &
   &
  \multicolumn{2}{c|}{$10^{-6}$} &
  \multicolumn{2}{c}{$10^{-5}$} \\ \cline{4-7} \cline{9-12} 
 &
   &
   &
  \multicolumn{1}{c|}{\textbf{FMs}} &
  \multicolumn{1}{c|}{\textbf{Weights}} &
  \multicolumn{1}{c|}{\textbf{FMs}} &
  \textbf{Weights} &
   &
  \multicolumn{1}{c|}{\textbf{FMs}} &
  \multicolumn{1}{c|}{\textbf{Weights}} &
  \multicolumn{1}{c|}{\textbf{FMs}} &
  \textbf{Weights} \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}BER \\ (DNN\\ level)\end{tabular}}}} &
  \multicolumn{1}{c|}{Baseline} &
  \multicolumn{1}{c|}{81.28\%} &
  \multicolumn{1}{c|}{71.24\%} &
  \multicolumn{1}{c|}{76.44\%} &
  \multicolumn{1}{c|}{67.36\%} &
  \multicolumn{1}{c|}{\textcolor{red}{66.56\%}} &
  \multicolumn{1}{c|}{88.14\%} &
  \multicolumn{1}{c|}{76.81\%} &
  \multicolumn{1}{c|}{65.79\%} &
  \multicolumn{1}{c|}{73.99\%} &
  30.66\% \\ \cline{2-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}} &
  \multicolumn{1}{c|}{76.40\%} &
  \multicolumn{1}{c|}{55.63\%} &
  \multicolumn{1}{c|}{73.75\%} &
  \multicolumn{1}{c|}{\textcolor{red}{51.28\%}} &
  \multicolumn{1}{c|}{72.45\%} &
  \multicolumn{1}{c|}{84.13\%} &
  \multicolumn{1}{c|}{76.14\%} &
  \multicolumn{1}{c|}{70.83\%} &
  \multicolumn{1}{c|}{75.96\%} &
  41.26\% \\ \cline{2-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}} &
  \multicolumn{1}{c|}{82.46\%} &
  \multicolumn{1}{c|}{66.20\%} &
  \multicolumn{1}{c|}{81.12\%} &
  \multicolumn{1}{c|}{58.66\%} &
  \multicolumn{1}{c|}{\textcolor{green}{80.63\%}} &
  \multicolumn{1}{c|}{72.80\%} &
  \multicolumn{1}{c|}{71.21\%} &
  \multicolumn{1}{c|}{61.11\%} &
  \multicolumn{1}{c|}{\textcolor{red}{70.97\%}} &
  \textcolor{red}{30.64\%} \\ \cline{2-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{Ranger} &
  \multicolumn{1}{c|}{81.28\%} &
  \multicolumn{1}{c|}{71.60\%} &
  \multicolumn{1}{c|}{76.88\%} &
  \multicolumn{1}{c|}{\textcolor{green}{68.08\%}} &
  \multicolumn{1}{c|}{69.37\%} &
  \multicolumn{1}{c|}{88.14\%} &
  \multicolumn{1}{c|}{80.57\%} &
  \multicolumn{1}{c|}{74.86\%} &
  \multicolumn{1}{c|}{\textcolor{green}{80.37\%}} &
  \textcolor{green}{43.92\%} \\ \cline{4-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c}{} &
  \multicolumn{1}{c|}{\textbf{Regs}} &
  \multicolumn{1}{c|}{\textbf{FUs}} &
  \multicolumn{1}{c|}{\textbf{Regs}} &
  \multicolumn{1}{c|}{\textbf{FUs}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{Regs}} &
  \multicolumn{1}{c|}{\textbf{FUs}} &
  \multicolumn{1}{c|}{\textbf{Regs}} &
  \textbf{FUs} \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Single \\ stuck-at\\ (ISA)\end{tabular}}}} &
  \multicolumn{1}{c|}{Baseline} &
  \multicolumn{1}{c|}{81.28\%} &
  \multicolumn{1}{c|}{72.99\%} &
  \multicolumn{1}{c|}{58.34\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} &
  \multicolumn{1}{c|}{\textcolor{red}{34.32\%}} &
  \multicolumn{1}{c|}{88.14\%} &
  \multicolumn{1}{c|}{\textcolor{green}{87.08\%}} &
  \multicolumn{1}{c|}{80.28\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}} &
  67.27\% \\ \cline{2-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}} &
  \multicolumn{1}{c|}{84.13\%} &
  \multicolumn{1}{c|}{72.18\%} &
  \multicolumn{1}{c|}{66.24\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}} &
  \multicolumn{1}{c|}{49.11\%} &
  \multicolumn{1}{c|}{84.13\%} &
  \multicolumn{1}{c|}{81.31\%} &
  \multicolumn{1}{c|}{77.10\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}} &
  50.35\% \\ \cline{2-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}} &
  \multicolumn{1}{c|}{72.80\%} &
  \multicolumn{1}{c|}{\textcolor{red}{71.59\%}} &
  \multicolumn{1}{c|}{62.62\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}} &
  \multicolumn{1}{c|}{60.63\%} &
  \multicolumn{1}{c|}{72.80\%} &
  \multicolumn{1}{c|}{\textcolor{red}{71.75\%}} &
  \multicolumn{1}{c|}{65.94\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}} &
  \textcolor{green}{71.70\%} \\ \cline{2-12} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{Ranger} &
  \multicolumn{1}{c|}{81.28\%} &
  \multicolumn{1}{c|}{\textcolor{green}{77.96\%}} &
  \multicolumn{1}{c|}{75.15\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}} &
  \multicolumn{1}{c|}{\textcolor{green}{68.47\%}} &
  \multicolumn{1}{c|}{88.14\%} &
  \multicolumn{1}{c|}{81.62\%} &
  \multicolumn{1}{c|}{81.95\%} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} - \end{tabular}} &
  \textcolor{red}{42.53\%} \\ \hline
\end{tabular}

\label{tab:colored_complete_table}
\end{table*}

==> tables/complete_mobilenet_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{ccccccccc}
\hline
\multicolumn{9}{c}{\textbf{Mobilenet V2}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multirow{3}{*}{\textbf{Fault model}}                                                                                  & \multirow{3}{*}{\textbf{Weights}}                                               & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} & \multicolumn{6}{c}{\textbf{Bit Error Rate}}                                                                                                                                                                                                                                                                                                                     \\ \cline{4-9} 
                                                                                                                       &                                                                                 &                                                                                      & \multicolumn{2}{c|}{$10^{-6}$}                                             & \multicolumn{2}{c|}{$10^{-5}$}                                                                                       & \multicolumn{2}{c|}{$10^{-4}$}                                                                                                                              \\ \cline{4-9} 
                                                                                                                       &                                                                                 &                                                                                      & \multicolumn{1}{c|}{\textbf{FMs}}  & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{FMs}}                                            & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{FMs}}                                            & \multicolumn{1}{c|}{\textbf{Weights}}                                        \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}BER\\ (Application\\ level)\end{tabular}}}}    & \multicolumn{1}{c|}{Baseline}                                                   & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{71.24\%}       & \multicolumn{1}{c|}{76.44\%}          & \multicolumn{1}{c|}{67.36\%}                                                 & \multicolumn{1}{c|}{66.56\%}          & \multicolumn{1}{c|}{59.18\%}                                                 & \multicolumn{1}{c|}{44.79\%}                                                 \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Clipper\end{tabular}} & \multicolumn{1}{c|}{76.40\%}                                                         & \multicolumn{1}{c|}{55.63\%}       & \multicolumn{1}{c|}{73.75\%}          & \multicolumn{1}{c|}{51.28\%}                                                 & \multicolumn{1}{c|}{72.45\%}          & \multicolumn{1}{c|}{46.07\%}                                                 & \multicolumn{1}{c|}{69.87\%}                                                 \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}      & \multicolumn{1}{c|}{82.46 \%}                                                        & \multicolumn{1}{c|}{66.20\%}       & \multicolumn{1}{c|}{84.12\%}          & \multicolumn{1}{c|}{58.66\%}                                                 & \multicolumn{1}{c|}{83.63\%}          & \multicolumn{1}{c|}{52.23\%}                                                 & \multicolumn{1}{c|}{80.99\%}                                                 \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{1}{c|}{Ranger}                                                     & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{71.60\%}       & \multicolumn{1}{c|}{76.88\%}          & \multicolumn{1}{c|}{68.08\%}                                                 & \multicolumn{1}{c|}{69.37\%}          & \multicolumn{1}{c|}{63.87}                                                   & \multicolumn{1}{c|}{53.87\%}                                                 \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{2}{c|}{}                                                                                                                                                  & \multicolumn{1}{c|}{\textbf{Regs}} & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{Regs}}                                           & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{Regs}}                                           & \multicolumn{1}{c|}{\textbf{FUs}}                                            \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Single bit-flips\\ (ISA-level)\end{tabular}}}} & \multicolumn{1}{c|}{Baseline}                                                   & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{72.99\%}       & \multicolumn{1}{c|}{58.34\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{34.32\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Clipper\end{tabular}} & \multicolumn{1}{c|}{76.40\%}                                                         & \multicolumn{1}{c|}{72.18\%}       & \multicolumn{1}{c|}{66.24\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{49.11\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}      & \multicolumn{1}{c|}{82.46 \%}                                                        & \multicolumn{1}{c|}{71.59\%}       & \multicolumn{1}{c|}{62.62\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{60.63\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                                 & \multicolumn{1}{c|}{Ranger}                                                     & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{77.96\%}       & \multicolumn{1}{c|}{75.15\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{68.47\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}

==> tables/complete_resnet_results.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{4}{*}{\textbf{Fault model}}                                                                                                 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hardening \\ Strategy\end{tabular}}} & \multicolumn{7}{c}{\textbf{Resnet18}}                                                                                                                                                                                                                                                                                          \\ \cmidrule(l){3-9} 
                                                                                                                                      &                                                                                         & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} & \multicolumn{6}{c}{\textbf{Bit Error Rate}}                                                                                                                                                                                             \\ \cmidrule(l){4-9} 
                                                                                                                                      &                                                                                         &                                                                                      & \multicolumn{2}{c|}{$10^{-6}$}                                                     & \multicolumn{2}{c|}{$10^{-5}$}                                                     & \multicolumn{2}{c}{$10^{-4}$}                                 \\ \cmidrule(l){4-9} 
                                                                                                                                      &                                                                                         &                                                                                      & \multicolumn{1}{c|}{\textbf{Feature maps}} & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{Feature maps}} & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{Feature maps}} & \textbf{Weights} \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Multiple bit-flips at \\ the Application-level\end{tabular}}}} & \multicolumn{1}{c|}{Baseline}                                                           & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{76.81\%}               & \multicolumn{1}{c|}{65.79\%}          & \multicolumn{1}{c|}{73.99\%}               & \multicolumn{1}{c|}{30.66\%}          & \multicolumn{1}{c|}{72.64\%}               & 14.71\%          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}}        & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{76.14\%}               & \multicolumn{1}{c|}{70.83\%}          & \multicolumn{1}{c|}{75.96\%}               & \multicolumn{1}{c|}{41.26\%}          & \multicolumn{1}{c|}{75.88\%}               & 17.63\%          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}              & \multicolumn{1}{c|}{72.80 \%}                                                        & \multicolumn{1}{c|}{71.21\%}               & \multicolumn{1}{c|}{61.11\%}          & \multicolumn{1}{c|}{70.97\%}               & \multicolumn{1}{c|}{30.64\%}          & \multicolumn{1}{c|}{70.86\%}               & 19.10\%          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{1}{c|}{Ranger}                                                             & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{80.57\%}               & \multicolumn{1}{c|}{74.86\%}          & \multicolumn{1}{c|}{80.37\%}               & \multicolumn{1}{c|}{43.92\%}          & \multicolumn{1}{c|}{80.28\%}               & 18.76\%          \\ \cmidrule(lr){2-2} \cmidrule(l){4-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{2}{c}{}                                                                                                                                                           & \multicolumn{1}{c|}{\textbf{Registers}}    & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{Registers}}    & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{Registers}}    & \textbf{FUs}     \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Single bit-flips at\\ the ISA-level\end{tabular}}}}            & \multicolumn{1}{c|}{Baseline}                                                           & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{87.86\%}               & \multicolumn{1}{c|}{77.67\%}          & \multicolumn{1}{c|}{Not generated}         & \multicolumn{1}{c|}{Not generated}    & \multicolumn{1}{c|}{Not generated}         & Not generated    \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}}        & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{84.13\%}               & \multicolumn{1}{c|}{75.64\%}          & \multicolumn{1}{c|}{Not generated}         & \multicolumn{1}{c|}{Not generated}    & \multicolumn{1}{c|}{Not generated}         & Not generated    \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}              & \multicolumn{1}{c|}{72.80 \%}                                                        & \multicolumn{1}{c|}{71.34\%}               & \multicolumn{1}{c|}{63.41\%}          & \multicolumn{1}{c|}{Not generated}         & \multicolumn{1}{c|}{Not generated}    & \multicolumn{1}{c|}{Not generated}         & Not generated    \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                                                                 & \multicolumn{1}{c|}{Ranger}                                                             & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{87.86\%}               & \multicolumn{1}{c|}{83.59\%}          & \multicolumn{1}{c|}{Not generated}         & \multicolumn{1}{c|}{Not generated}    & \multicolumn{1}{c|}{Not generated}         & Not generated    \\ \cmidrule(l){2-9} 
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table*}


==> tables/complete_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{7}{c|}{\textbf{Mobilenet V2}}                                                                                                                                                                                                                                                                                                                                                                                                                                                        & \multicolumn{5}{c}{\textbf{Resnet 18}}                                                                                                                                                                                                                             \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fault\\ model\end{tabular}}}                                   & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hardening\\ Strategy\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} & \multicolumn{4}{c}{\textbf{Bit Error Rate}}                                                                                                                                                   & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} & \multicolumn{4}{c}{Bit Error Rate}                                                                                                                                          \\ \cline{4-7} \cline{9-12} 
                                                                                                                  &                                                                                        &                                                                                      & \multicolumn{2}{c|}{$10^{-6}$}                                             & \multicolumn{2}{c}{$10^{-5}$}                                                                                    &                                                                                      & \multicolumn{2}{c|}{$10^{-6}$}                                             & \multicolumn{2}{c}{$10^{-5}$}                                                                  \\ \cline{4-7} \cline{9-12} 
                                                                                                                  &                                                                                        &                                                                                      & \multicolumn{1}{c|}{\textbf{FMs}}  & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{FMs}}                                            & \textbf{Weights}                  &                                                                                      & \multicolumn{1}{c|}{\textbf{FMs}}  & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{FMs}}                                           & \textbf{Weights} \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}BER \\ (DNN\\ level)\end{tabular}}}}       & \multicolumn{1}{c|}{Baseline}                                                          & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{71.24\%}       & \multicolumn{1}{c|}{76.44\%}          & \multicolumn{1}{c|}{67.36\%}                                                 & \multicolumn{1}{c|}{66.56\%}      & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{76.81\%}       & \multicolumn{1}{c|}{65.79\%}          & \multicolumn{1}{c|}{73.99\%}                                                & 30.66\%          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}}       & \multicolumn{1}{c|}{76.40\%}                                                         & \multicolumn{1}{c|}{55.63\%}       & \multicolumn{1}{c|}{73.75\%}          & \multicolumn{1}{c|}{51.28\%}                                                 & \multicolumn{1}{c|}{72.45\%}      & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{76.14\%}       & \multicolumn{1}{c|}{70.83\%}          & \multicolumn{1}{c|}{75.96\%}                                                & 41.26\%          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}             & \multicolumn{1}{c|}{82.46\%}                                                         & \multicolumn{1}{c|}{66.20\%}       & \multicolumn{1}{c|}{84.12\%}          & \multicolumn{1}{c|}{58.66\%}                                                 & \multicolumn{1}{c|}{83.63\%}      & \multicolumn{1}{c|}{72.80\%}                                                         & \multicolumn{1}{c|}{71.21\%}       & \multicolumn{1}{c|}{61.11\%}          & \multicolumn{1}{c|}{70.97\%}                                                & 30.64\%          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{Ranger}                                                            & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{71.60\%}       & \multicolumn{1}{c|}{76.88\%}          & \multicolumn{1}{c|}{68.08\%}                                                 & \multicolumn{1}{c|}{69.37\%}      & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{80.57\%}       & \multicolumn{1}{c|}{74.86\%}          & \multicolumn{1}{c|}{80.37\%}                                                & 43.92\%          \\ \cline{4-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{2}{c}{}                                                                                                                                                          & \multicolumn{1}{c|}{\textbf{Regs}} & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{Regs}}                                           & \multicolumn{1}{c|}{\textbf{FUs}} & \multicolumn{1}{c|}{}                                                                & \multicolumn{1}{c|}{\textbf{Regs}} & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{Regs}}                                          & \textbf{FUs}     \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Single \\ stuck-at\\ (ISA)\end{tabular}}}} & \multicolumn{1}{c|}{Baseline}                                                          & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{72.99\%}       & \multicolumn{1}{c|}{58.34\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ activated\end{tabular}} & \multicolumn{1}{c|}{34.32\%}      & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{87.08\%}       & \multicolumn{1}{c|}{80.28\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 67.27\%          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}}       & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{72.18\%}       & \multicolumn{1}{c|}{66.24\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}}  & \multicolumn{1}{c|}{49.11\%}      & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{81.31\%}       & \multicolumn{1}{c|}{77.10\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 50.35\%          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}             & \multicolumn{1}{c|}{72.80 \%}                                                        & \multicolumn{1}{c|}{71.59\%}       & \multicolumn{1}{c|}{62.62\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}}  & \multicolumn{1}{c|}{60.63\%}      & \multicolumn{1}{c|}{72.80\%}                                                         & \multicolumn{1}{c|}{71.75\%}       & \multicolumn{1}{c|}{65.94\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 71.70\%          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{Ranger}                                                            & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{77.96\%}       & \multicolumn{1}{c|}{75.15\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}}  & \multicolumn{1}{c|}{68.47\%}      & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{81.62\%}       & \multicolumn{1}{c|}{81.95\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 42.53\%          \\ \hline
\end{tabular}
\caption{}
\label{tab:complete_table}
\end{table*}

==> tables/minimal_mobilenet_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Accuracy of the Baseline model (Mobilenet V2) and of the model with application level hardening techniques. A comparison between multipl}
\begin{tabular}{ccccccc}
\hline
\multicolumn{7}{c}{\textbf{Mobilenet V2}}                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fault \\ model\end{tabular}}}                                   & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hardening\\ Strategy\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} & \multicolumn{4}{c}{\textbf{Bit Error Rate}}                                                                                                                                  \\ \cline{4-7} 
                                                                                                                   &                                                                                        &                                                                                      & \multicolumn{2}{c|}{$10^{-6}$}                                             & \multicolumn{2}{c}{$10^{-5}$}                                                                   \\ \cline{4-7} 
                                                                                                                   &                                                                                        &                                                                                      & \multicolumn{1}{c|}{\textbf{FMs}}  & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{FMs}}                                            & \textbf{Weights} \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}BER\\ (DNN\\ level)\end{tabular}}}}       & \multicolumn{1}{c|}{Baseline}                                                          & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{71.24\%}       & \multicolumn{1}{c|}{76.44\%}          & \multicolumn{1}{c|}{67.36\%}                                                 & 66.56\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Clipper\end{tabular}}        & \multicolumn{1}{c|}{76.40\%}                                                         & \multicolumn{1}{c|}{55.63\%}       & \multicolumn{1}{c|}{73.75\%}          & \multicolumn{1}{c|}{51.28\%}                                                 & 72.45\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}             & \multicolumn{1}{c|}{82.46 \%}                                                        & \multicolumn{1}{c|}{66.20\%}       & \multicolumn{1}{c|}{84.12\%}          & \multicolumn{1}{c|}{58.66\%}                                                 & 83.63\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{Ranger}                                                            & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{71.60\%}       & \multicolumn{1}{c|}{76.88\%}          & \multicolumn{1}{c|}{68.08\%}                                                 & 69.37\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{2}{c|}{}                                                                                                                                                         & \multicolumn{1}{c|}{\textbf{RFs}} & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{RFs}}                                           & \textbf{FUs}     \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Single \\ stuck-at faults\\ (ISA)\end{tabular}}}} & \multicolumn{1}{c|}{Baseline}                                                          & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{72.99\%}       & \multicolumn{1}{c|}{58.34\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 34.32\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Clipper\end{tabular}}        & \multicolumn{1}{c|}{76.40\%}                                                         & \multicolumn{1}{c|}{72.18\%}       & \multicolumn{1}{c|}{66.24\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 49.11\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}             & \multicolumn{1}{c|}{82.46 \%}                                                        & \multicolumn{1}{c|}{71.59\%}       & \multicolumn{1}{c|}{62.62\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 60.63\%          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{Ranger}                                                            & \multicolumn{1}{c|}{81.28\%}                                                         & \multicolumn{1}{c|}{77.96\%}       & \multicolumn{1}{c|}{75.15\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & 68.47\%          \\ \hline
\end{tabular}

\label{tab:mobilenet}
\end{table*}

==> tables/minmal_resnet_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{ccccccc}
\hline
\multicolumn{7}{c}{\textbf{Resnet18}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fault\\ model\end{tabular}}}                                   & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hardening\\ Strategy\end{tabular}}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Golden \\ accuracy\end{tabular}}} & \multicolumn{4}{c}{\textbf{Bit Error Rate}}                                                                                                                                                       \\ \cline{4-7} 
                                                                                                                  &                                                                                        &                                                                                      & \multicolumn{2}{c|}{$10^{-6}$}                                             & \multicolumn{2}{c|}{$10^{-5}$}                                                                                       \\ \cline{4-7} 
                                                                                                                  &                                                                                        &                                                                                      & \multicolumn{1}{c|}{\textbf{FMs}}  & \multicolumn{1}{c|}{\textbf{Weights}} & \multicolumn{1}{c|}{\textbf{FMs}}                                            & \multicolumn{1}{c|}{\textbf{Weights}} \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}BER \\ (DNN\\ level)\end{tabular}}}}       & \multicolumn{1}{c|}{Baseline}                                                          & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{76.81\%}       & \multicolumn{1}{c|}{65.79\%}          & \multicolumn{1}{c|}{73.99\%}                                                 & \multicolumn{1}{c|}{30.66\%}          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}}       & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{76.14\%}       & \multicolumn{1}{c|}{70.83\%}          & \multicolumn{1}{c|}{75.96\%}                                                 & \multicolumn{1}{c|}{41.26\%}          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}             & \multicolumn{1}{c|}{72.80 \%}                                                        & \multicolumn{1}{c|}{71.21\%}       & \multicolumn{1}{c|}{61.11\%}          & \multicolumn{1}{c|}{70.97\%}                                                 & \multicolumn{1}{c|}{30.64\%}          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{Ranger}                                                            & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{80.57\%}       & \multicolumn{1}{c|}{74.86\%}          & \multicolumn{1}{c|}{80.37\%}                                                 & \multicolumn{1}{c|}{43.92\%}          \\ \cline{4-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{2}{c}{}                                                                                                                                                          & \multicolumn{1}{c|}{\textbf{RFs}} & \multicolumn{1}{c|}{\textbf{FUs}}     & \multicolumn{1}{c|}{\textbf{RFs}}                                           & \multicolumn{1}{c|}{\textbf{FUs}}     \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Single \\ stuck-at\\ (ISA)\end{tabular}}}} & \multicolumn{1}{c|}{Baseline}                                                          & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{87.08\%}       & \multicolumn{1}{c|}{80.28\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & \multicolumn{1}{c|}{67.27\%}          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}}       & \multicolumn{1}{c|}{84.13\%}                                                         & \multicolumn{1}{c|}{81.31\%}       & \multicolumn{1}{c|}{77.10\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & \multicolumn{1}{c|}{50.35\%}          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}}             & \multicolumn{1}{c|}{72.80 \%}                                                        & \multicolumn{1}{c|}{71.75\%}       & \multicolumn{1}{c|}{65.94\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & \multicolumn{1}{c|}{71.70\%}          \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{Ranger}                                                            & \multicolumn{1}{c|}{88.14\%}                                                         & \multicolumn{1}{c|}{81.62\%}       & \multicolumn{1}{c|}{81.95\%}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Not\\ observed\end{tabular}} & \multicolumn{1}{c|}{42.53\%}          \\ \cline{2-7} 
\end{tabular}
\caption{}
\label{tab:resnet}
\end{table*}

==> tables/transposed_colored_complete_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Accuracy (in percentage) for the baseline DNNs and their hardened versions. The simulation results are obtained by corrupting DNNs parameters (BER, DNN-level) and basic instructions (Single stuck-at, ISA-level). 
For each FI campaign, the worst and the best accuracy scores are highlighted in red and in green, respectively.}
\begin{tabular}{c|ccc|ccccc|cccc}
\hline
\textbf{} &
  \multicolumn{3}{c|}{\textbf{Fault model}} &
  \multicolumn{5}{c|}{\textbf{BER (DNN-level)}} &
  \multicolumn{4}{c}{\textbf{Single stuck-at (ISA-level)}} \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{c|}{\textbf{Hardening Strategy}} &
  \multicolumn{1}{c|}{Baseline} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}} &
  \multicolumn{1}{c|}{Ranger} &
  \multirow{2}{*}{} &
  \multicolumn{1}{c|}{Baseline} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive \\ Clipper\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swap \\ ReLU6\end{tabular}} &
  Ranger \\ \cline{1-8} \cline{10-13} 
\multicolumn{1}{l|}{\multirow{5}{*}{\textbf{Mobilenet V2}}} &
  \multicolumn{3}{c|}{\textbf{Golden accuracy}} &
  \multicolumn{1}{c|}{81.28\%} &
  \multicolumn{1}{c|}{76.40\%} &
  \multicolumn{1}{c|}{82.46\%} &
  \multicolumn{1}{c|}{81.28\%} &
   &
  \multicolumn{1}{c|}{81.28\%} &
  \multicolumn{1}{c|}{84.13\%} &
  \multicolumn{1}{c|}{72.80\%} &
  81.28\% \\ \cline{2-13} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Neurons}}} &
  \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{BER}}} &
  $10^{-6}$ &
  \multicolumn{1}{c|}{71.24\%} &
  \multicolumn{1}{c|}{55.63\%} &
  \multicolumn{1}{c|}{66.20\%} &
  \multicolumn{1}{c|}{71.60\%} &
  \multirow{2}{*}{\textbf{Regs}} &
  \multicolumn{1}{c|}{72.99\%} &
  \multicolumn{1}{c|}{72.18\%} &
  \multicolumn{1}{c|}{\textcolor{red}{71.59\%}} &
  \textcolor{green}{77.96\%} \\ \cline{4-8} \cline{10-13} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  $10^{-5}$ &
  \multicolumn{1}{c|}{67.36\%} &
  \multicolumn{1}{c|}{\textcolor{red}{51.28\%}} &
  \multicolumn{1}{c|}{58.66\%} &
  \multicolumn{1}{c|}{\textcolor{green}{68.08\%}} &
   &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Weights}}} &
  \multicolumn{1}{c|}{} &
  $10^{-6}$ &
  \multicolumn{1}{c|}{76.44\%} &
  \multicolumn{1}{c|}{73.75\%} &
  \multicolumn{1}{c|}{84.12\%} &
  \multicolumn{1}{c|}{76.88\%} &
  \multirow{2}{*}{\textbf{FUs}} &
  \multicolumn{1}{c|}{58.34\%} &
  \multicolumn{1}{c|}{66.24\%} &
  \multicolumn{1}{c|}{62.62\%} &
  75.15\% \\ \cline{4-8} \cline{10-13} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  $10^{-5}$ &
  \multicolumn{1}{c|}{\textcolor{red}{66.56\%}} &
  \multicolumn{1}{c|}{72.45\%} &
  \multicolumn{1}{c|}{\textcolor{green}{81.63\%}} &
  \multicolumn{1}{c|}{69.37\%} &
   &
  \multicolumn{1}{c|}{\textcolor{red}{34.32\%}} &
  \multicolumn{1}{c|}{49.11\%} &
  \multicolumn{1}{c|}{60.63\%} &
  \textcolor{green}{68.47\%} \\ \hline
\multirow{5}{*}{\textbf{Resnet18}} &
  \multicolumn{3}{c|}{\textbf{Golden accuracy}} &
  \multicolumn{1}{c|}{88.14\%} &
  \multicolumn{1}{c|}{84.13\%} &
  \multicolumn{1}{c|}{72.80\%} &
  \multicolumn{1}{c|}{88.14\%} &
   &
  \multicolumn{1}{c|}{88.14\%} &
  \multicolumn{1}{c|}{84.13\%} &
  \multicolumn{1}{c|}{72.80\%} &
  88.14\% \\ \cline{2-13} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Neurons}}} &
  \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{BER}}} &
  $10^{-6}$ &
  \multicolumn{1}{c|}{76.81\%} &
  \multicolumn{1}{c|}{76.14\%} &
  \multicolumn{1}{c|}{71.21\%} &
  \multicolumn{1}{c|}{80.57\%} &
  \multirow{2}{*}{\textbf{Regs}} &
  \multicolumn{1}{c|}{\textcolor{green}{87.08\%}} &
  \multicolumn{1}{c|}{81.31\%} &
  \multicolumn{1}{c|}{\textcolor{red}{71.75\%}} &
  81.62\% \\ \cline{4-8} \cline{10-13} 
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  $10^{-5}$ &
  \multicolumn{1}{c|}{73.99\%} &
  \multicolumn{1}{c|}{75.96\%} &
  \multicolumn{1}{c|}{\textcolor{red}{70.97\%}} &
  \multicolumn{1}{c|}{\textcolor{green}{80.37\%}} &
   &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-2} \cline{4-13} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Weights}}} &
  \multicolumn{1}{c|}{} &
  $10^{-6}$ &
  \multicolumn{1}{c|}{65.79\%} &
  \multicolumn{1}{c|}{70.83\%} &
  \multicolumn{1}{c|}{61.11\%} &
  \multicolumn{1}{c|}{74.86\%} &
  \multirow{2}{*}{\textbf{FUs}} &
  \multicolumn{1}{c|}{80.28\%} &
  \multicolumn{1}{c|}{77.10\%} &
  \multicolumn{1}{c|}{65.94\%} &
  81.95\% \\ \cline{4-8} \cline{10-13} 
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  $10^{-5}$ &
  \multicolumn{1}{c|}{30.66\%} &
  \multicolumn{1}{c|}{41.26\%} &
  \multicolumn{1}{c|}{\textcolor{red}{30.64\%}} &
  \multicolumn{1}{c|}{\textcolor{green}{43.92\%}} &
   &
  \multicolumn{1}{c|}{67.27\%} &
  \multicolumn{1}{c|}{50.35\%} &
  \multicolumn{1}{c|}{\textcolor{green}{71.70\%}} &
  \textcolor{red}{42.53\%} \\ \hline
\multirow{5}{*}{\textbf{Lenet5}} &
  \multicolumn{3}{c|}{\textbf{Golden accuracy}} &
  \multicolumn{1}{c|}{98.00\%} &
  \multicolumn{1}{c|}{98.00\%} &
  \multicolumn{1}{c|}{98.25\%} &
  \multicolumn{1}{c|}{98.00\%} &
   &
  \multicolumn{1}{c|}{98.00\%} &
  \multicolumn{1}{c|}{98.00\%} &
  \multicolumn{1}{c|}{98.25\%} &
  98.00\% \\ \cline{2-13} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Neurons}}} &
  \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{BER}}} &
  $10^{-6}$ &
  \multicolumn{1}{c|}{83.60\%} &
  \multicolumn{1}{c|}{95.65\%} &
  \multicolumn{1}{c|}{93.19\%} &
  \multicolumn{1}{c|}{94.80\%} &
  \multirow{2}{*}{\textbf{Regs}} &
  \multicolumn{1}{c|}{\textcolor{green}{98.00\%}} &
  \multicolumn{1}{c|}{\textcolor{red}{97.10\%}} &
  \multicolumn{1}{c|}{97.23\%} &
  \textcolor{green}{98.00\%} \\ \cline{4-8} \cline{10-13} 
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  $10^{-5}$ &
  \multicolumn{1}{c|}{\textcolor{red}{75.12\%}} &
  \multicolumn{1}{c|}{\textcolor{green}{93.96\%}} &
  \multicolumn{1}{c|}{88.10\%} &
  \multicolumn{1}{c|}{93.55\%} &
   &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-2} \cline{4-13} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Weights}}} &
  \multicolumn{1}{c|}{} &
  $10^{-6}$ &
  \multicolumn{1}{c|}{95.37\%} &
  \multicolumn{1}{c|}{97.30\%} &
  \multicolumn{1}{c|}{94.70\%} &
  \multicolumn{1}{c|}{97.40\%} &
  \multirow{2}{*}{\textbf{FUs}} &
  \multicolumn{1}{c|}{93.55\%} &
  \multicolumn{1}{c|}{92.81\%} &
  \multicolumn{1}{c|}{87.09\%} &
  95.96\% \\ \cline{4-8} \cline{10-13} 
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  $10^{-5}$ &
  \multicolumn{1}{c|}{75.54\%} &
  \multicolumn{1}{c|}{\textcolor{green}{95.01\%}} &
  \multicolumn{1}{c|}{\textcolor{red}{76.35\%}} &
  \multicolumn{1}{c|}{93.50\%} &
   &
  \multicolumn{1}{c|}{\textcolor{red}{86.20\%}} &
  \multicolumn{1}{c|}{\textcolor{green}{91.63\%}} &
  \multicolumn{1}{c|}{90.51\%} &
  91.42\% \\ \hline
\end{tabular}

\label{tab:transposed_colored_complete_table}
\vspace{-7mm}
\end{table*}
